Graph fission and cross-validation

We introduce a technique called graph fission which takes in a graph which potentially contains only one observation per node (whose distribution lies in a known class) and produces two (or more) independent graphs with the same node/edge set in a way that splits the original graph's information amongst them in any desired proportion. Our proposal builds on data fission/thinning, a method that uses external randomization to create independent copies of an unstructured dataset. We extend this idea to the graph setting where there may be latent structure between observations. We demonstrate the utility of this framework via two applications: inference after structural trend estimation on graphs and a model selection procedure we term "graph cross-validation".

==> checklist.tex <==

\section*{Checklist}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [\emph{\textbf{Yes}}/No/Not Applicable]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes/No/\emph{\textbf{Not Applicable}}]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [\emph{\textbf{Yes}}/No/Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [\emph{\textbf{Yes}}/No/Not Applicable]
   \item Complete proofs of all theoretical results. [\emph{\textbf{Yes}}/No/Not Applicable]
   \item Clear explanations of any assumptions. [\emph{\textbf{Yes}}/No/Not Applicable]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [\emph{\textbf{Yes}}/No/Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [\emph{\textbf{Yes}}/No/Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [\emph{\textbf{Yes}}/No/Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [\emph{\textbf{Yes}}/No/Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [\emph{\textbf{Yes}}/No/Not Applicable]
   \item The license information of the assets, if applicable. [Yes/No/\emph{\textbf{Not Applicable}}]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes/No/\emph{\textbf{Not Applicable}}]
   \item Information about consent from data providers/curators. [\emph{\textbf{Yes}}/No/Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Yes/No/\emph{\textbf{Not Applicable}}]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Yes/No/\emph{\textbf{Not Applicable}}]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Yes/No/\emph{\textbf{Not Applicable}}]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Yes/No/\emph{\textbf{Not Applicable}}]
 \end{enumerate}

 \end{enumerate}


==> header.tex <==
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{epsf}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage[dvipsnames]{xcolor}

\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm}

\usepackage[utf8]{inputenc}
\usepackage[colorlinks=true, allcolors=blue]{hyperref}
\usepackage[authoryear]{natbib}
\usepackage{appendix}

\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\newsavebox{\bigimage}
\usepackage{multirow}
\usepackage{float}
\usepackage[nodisplayskipstretch]{setspace} 
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage{pifont}%
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\RequirePackage{forloop}
\RequirePackage{url}

\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Ima}{\mathrm{im}}
\newcommand{\Ker}{\mathrm{ker}}
\newcommand{\Rank}{\mathrm{rank}}
\newcommand{\Dim}{\mathrm{dim }}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}
\newcommand{\pos}{\mathrm{Pos}\xspace}
\newcommand{\me}{\mathbb{E}}
\newcommand{\one}{\mathds{1}\xspace}
\newcommand{\pei}{$\mathrm{I}^3$\xspace}
\newcommand{\peiZero}{Crossfit-$\mathrm{I}^3$\xspace}
\newcommand{\peiNeg}{MaY-$\mathrm{I}^3$\xspace}
\newcommand{\peiZeroKnowP}{Crossfit-$\mathrm{I}^3_{\pi^*}$\xspace}
\newcommand{\peiNegKnowP}{MaY-$\mathrm{I}^3_{\pi^*}$\xspace}
\newcommand{\peiZeroUnknowP}{Crossfit-$\mathrm{I}^3_{\widehat \pi}$\xspace}
\newcommand{\peiNegUnknowP}{MaY-$\mathrm{I}^3_{\widehat \pi}$\xspace}
\newcommand{\peiZeroUnknowY}{Crossfit-$\mathrm{I}^3_{\widehat Y}$\xspace}
\newcommand{\peiNegUnknowY}{MaY-$\mathrm{I}^3_{\widehat Y}$\xspace}

\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{fact}{Fact}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{setting}{Setting}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{property}{Property}

\newcommand{\independent}{\perp\mkern-9.5mu\perp}
\newcommand{\notindependent}{\centernot{\independent}}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

